Refutation calculi for lattice-based logics: from display to tableaux

Refutation calculi are formal systems developed to derive the invalid formulas of a given logic. While the notion of refutation calculi has played a key role in the development of tableaux calculi, a refutation approach to display calculi has not yet been attempted. In this paper, we introduce refutation display calculi for basic LE-logics, i.e., those logics canonically associated with basic normal lattice expansions of any signature. In particular, we prove soundness and completeness via proof-analysis results on derivable sequents. Finally, we obtain terminating tableaux calculi from these refutation display calculi.

==> ManagingDisplayEquivalence.tex <==
\section{Managing display-equivalence}
  The sequents $\Pi_i \vdash \Sigma_i$ for $1\leq i\leq 2$ are \emph{display equivalent} (notation: $\Pi_1 \vdash \Sigma_1 \equiv_D \Pi_2 \vdash \Sigma_2$) if they are interderivable via display postulates. 
  %Clearly, $\equiv_D$ is an equivalence relation.
  \textcolor{red}{Alessandra e Giuseppe: quando passate di qui scegliete quale versione della definizione 3 tenere. Vorrei che gli archi restassero labelled.}
\begin{definition} \label{def:sequent_tree} For any $\Upsilon \in \mathsf{Str}$, we let $\mathcal{T}(\Upsilon)$ denote the {\em generation tree} of $\Upsilon$, recursively defined as the generation tree of formulas, but taking arbitrary $\mathcal{L}_{\mathrm{LE}}$-formulas as the base case. %except that the leaves of $\mathcal{T}(\Upsilon)$ are the formulas in $\Upsilon$. 
The {\em positive} (resp.~{\em negative}) generation tree of $\Upsilon$ is obtained by decorating the root of $\mathcal{T}(\Upsilon)$ with a sign $+$ (resp.~$-$), and then propagating the decoration to each child node according to the order-type of its parent-node: same sign as the parent-node to the children corresponding to positive coordinates of the parent-node, opposite sign to those corresponding to negative ones.   The {\em (signed)} {\em generation tree} $\mathcal{T}(\Pi\vdash\Sigma)$  of a sequent $\Pi \vdash \Sigma$ is obtained by connecting the roots of (the positive tree) $\mathcal{T}(\Pi)$ and (the negative tree) $\mathcal{T}(\Sigma)$ with a new root, labelled `$\vdash$'.
  
    
    The   (rooted) tree $\mathcal{T}(\Upsilon)$ of any  $\Upsilon\in \mathsf{Str}$ is recursively defined  as follows.
    \begin{itemize}
        \item If $\Upsilon \coloneqq \varphi$ is a formula, $\mathcal{T}(\varphi)$ is a single vertex labelled `$\varphi$'.
        \item If $\Upsilon \coloneqq H(\Upsilon_1,\ldots,\Upsilon_n)$, where $H$ is a structural connective, $\mathcal{T}(\Pi)$ is
        \begin{center}
        \begin{forest}
[H
[$\mathcal{T}(\Upsilon_1)$, -->, edge label = {node [midway, above left, font = \scriptsize] {$1$}}]
%[$\cdots$, edge=dotted]
[$\mathcal{T}(\Upsilon_n)$, edge label = {node [midway, above right, font = \scriptsize] {$n$}}]
  ]
\end{forest} 
        \end{center}

\remove{
%edge label = {node [midway, above left, font = \scriptsize] {\textcolor{red}{$1$}}}
\begin{center}
\begin{tabular}{cc}
\begin{forest}
[H
    [$\mathcal{T}(\Upsilon_1)$, edge label = {node [midway, above left, font = \scriptsize] {$1$}}]
    [$\cdots$, no edge]
    [$\mathcal{T}(\Upsilon_n)$, edge label = {node [midway, above right, font = \scriptsize] {$n$}}]
  ]
\end{forest}
 &&
\begin{forest}
[H
    [$\mathcal{T}(\Upsilon_1)$, edge label = {node [midway, above left, font = \scriptsize] {$1$}}]
    [$\cdots$, edge=dotted]
    [$\mathcal{T}(\Upsilon_n)$, edge label = {node [midway, above right, font = \scriptsize] {$n$}}]
  ]
\end{forest} 
\\
\end{tabular}
\end{center}
}


%\begin{center}
%        \begin{forest}
%            for tree = {
%                circle, draw, 
%                minimum size=5em,
%                inner sep=4pt,
%            %
%                s sep=15mm,
%                l sep=20mm,
%                edge={-Straight Barb}, % arrows head defined in 'arrows.meta'
%                EL/.style = {edge label={node[midway, fill=white, inner sep=2pt,
%                                        anchor=center]{#1}},},
%                        }
%            [ItemA
%                [ItemB,EL=left]
%                [ItemC,EL=right]
%            ]
%        \end{forest}
%    \end



    \end{itemize}
    Given an arbitrary sequent $\Pi \vdash \Sigma$, the associated tree of $\Pi \vdash \Sigma$, denoted as $\mathcal{T}(\Pi\vdash\Sigma)$, is obtained by connecting the roots of $\mathcal{T}(\Pi)$ and $\mathcal{T}(\Sigma)$ with a new edge, labelled `$\vdash$'.

\end{definition}

\begin{lemma} \label{lem:tree_under_display_postulates}
The size of the equivalence class $[\Pi \vdash \Sigma]_{\equiv_D}$ is exactly the number of edges of $\mathcal{T}(\Pi\vdash\Sigma)$. Furthermore, the unlabelled versions of the associated trees of every member of $[\Pi \vdash \Sigma]_{\equiv_D}$ are isomorphic.
\end{lemma}
\begin{proof}
To understand the effect of display postulates on $\mathcal{T}(\Pi \vdash \Sigma)$, we consider the cases where the structural connective to be residuated occurs in $\Pi$ (those for $\Sigma$ are analogous), assuming $\Pi = \FH(\Upsilon_1, \ldots, \Pi_i, \ldots, \Upsilon_n)$. When $\varepsilon_f(i) = 1$, %We need to understand how $\mathcal{T}(\Pi\vdash\Sigma)$ changes when display postulates are applied to the sequent $\Pi\vdash\Sigma$. Below we show the cases where the structural connective to residuate is in $\Pi$ (the cases in $\Sigma$ being analogous), and $\Pi=\FH(\Upsilon_1, \ldots, \Pi_i, \ldots, \Upsilon_1)$. When $\varepsilon_f(i)=1$,
\begin{center}
\begin{tabular}{c c c}
     \begin{tikzpicture}
            \node (Lparent) {$\FH$}
                child{node (child1) {$\mathcal{T}(\Upsilon_1)$}
                edge from parent node[left] {1}
                edge from parent node[right] {$\cdots$}
                }
                child{node (childi) {$\mathcal{T}(\Pi_i)$}
                %edge from parent node[left] {1}
                edge from parent node[right] {$\cdots$}
                }
                child{node (childn) {$\mathcal{T}(\Upsilon_{n_f})$}
                edge from parent node[right] {$n_f$}
                };
                \node[right=2cm of Lparent] (Rparent) {$\mathcal{T}(\Sigma)$};
                \draw (Lparent) -- node[above] {$\vdash$} (Rparent);
        \end{tikzpicture}
     &
     $\xLeftrightarrow{\FH \vdash \FCS_i}$
     &
     \begin{tikzpicture}
     \node (Lparent) {$\mathcal{T}(\Pi_i)$};
                
            \node[right=2cm of Lparent] (Rparent) {$\FCS_i$}
                child{node (child1) {$\mathcal{T}(\Upsilon_1)$}
                edge from parent node[left] {1}
                edge from parent node[right] {$\cdots$}
                }
                child{node (childi) {$\mathcal{T}(\Sigma)$}
                %edge from parent node[left] {1}
                edge from parent node[right] {$\cdots$}
                }
                child{node (childn) {$\mathcal{T}(\Upsilon_{n_f})$}
                edge from parent node[right] {$n_f$}
                };
                \draw (Lparent) -- node[above] {$\vdash$} (Rparent);
        \end{tikzpicture}
     \end{tabular}
     \end{center}

\remove{
\textcolor{red}{GG: Below I draw the sequent generation trees (see Definition \ref{def:sequent_tree}) using forest:
%
\begin{center}
\begin{tikzpicture}
\node (left) at (-3,0) { 
\begin{forest}
[$\vdash$
[$\FH$
[$\mathcal{T}(\Upsilon_1)$, -->, edge label = {node [midway, above left, font = \scriptsize] {$1$}}]
%[$\cdots$, no edge]
[$\mathcal{T}(\Pi_i)$, -->, edge label = {node [midway, right, font = \scriptsize] {$i$}}]
%[$\cdots$, no edge] 
[$\mathcal{T}(\Upsilon_{n_f})$, edge label = {node [midway, above right, font = \scriptsize] {$n_f$}}]]
[$\mathcal{T}(\Sigma)$ [ \ \ \ , no edge]] 
]
%\draw[-,dotted](1)..(i);
\end{forest}};
%
\node (iff) at (0,1.2) {$\xLeftrightarrow{\FH \vdash \FCS_i}$};
%
\node (right) at (3,0) {
\begin{forest}
[$\vdash$
[$\mathcal{T}(\Pi_i)$ [ \ \ \ , no edge]] 
[$\FCS_i$
[$\mathcal{T}(\Upsilon_1)$, -->, edge label = {node [midway, above left, font = \scriptsize] {$1$}}]
%[$\cdots$, no edge]
[$\mathcal{T}(\Sigma)$, -->, edge label = {node [midway, right, font = \scriptsize] {$i$}}]
%[$\cdots$, no edge]
[$\mathcal{T}(\Upsilon_{n_f})$, edge label = {node [midway, above right, font = \scriptsize] {$n_f$}}]]
]
\end{forest}};
\end{tikzpicture}
\end{center}
}}

\noindent and when $\varepsilon_f(i)=\partial$
     \begin{center}
    \begin{tabular}{c c c}
     \begin{tikzpicture}
            \node (Lparent) {$\FH$}
                child{node (child1) {$\mathcal{T}(\Upsilon_1)$}
                edge from parent node[left] {1}
                edge from parent node[right] {$\cdots$}
                }
                child{node (childi) {$\mathcal{T}(\Sigma_i)$}
                %edge from parent node[left] {1}
                edge from parent node[right] {$\cdots$}
                }
                child{node (childn) {$\mathcal{T}(\Upsilon_{n_f})$}
                edge from parent node[right] {$n_f$}
                };
                \node[right=2cm of Lparent] (Rparent) {$\mathcal{T}(\Sigma)$};
                \draw (Lparent) -- node[above] {$\vdash$} (Rparent);
        \end{tikzpicture}
     &
     $\xLeftrightarrow{(\FH, \FHS_i)}$
     &
     \begin{tikzpicture}
            \node (Lparent) {$\FHS_i$}
                child{node (child1) {$\mathcal{T}(\Upsilon_1)$}
                edge from parent node[left] {1}
                edge from parent node[right] {$\cdots$}
                }
                child{node (childi) {$\mathcal{T}(\Sigma)$}
                %edge from parent node[left] {1}
                edge from parent node[right] {$\cdots$}
                }
                child{node (childn) {$\mathcal{T}(\Upsilon_{n_f})$}
                edge from parent node[right] {$n_f$}
                };
                \node[right=2cm of Lparent] (Rparent) {$\mathcal{T}(\Sigma_i)$};
                \draw (Lparent) -- node[above] {$\vdash$} (Rparent);
        \end{tikzpicture}
\end{tabular}
\end{center}

\remove{\textcolor{red}{GG: Below I draw the sequent generation trees (see Definition \ref{def:sequent_tree}) using forest:
%
\begin{center}
\begin{tikzpicture}
\node (left) at (-3,0) { 
\begin{forest}
[$\vdash$
[$\FH$
[$\mathcal{T}(\Upsilon_1)$, -->, edge label = {node [midway, above left, font = \scriptsize] {$1$}}]
%
[$\mathcal{T}(\Sigma_i)$, -->, edge label = {node [midway, right, font = \scriptsize] {$i$}}]
%
[$\mathcal{T}(\Upsilon_{n_f})$, edge label = {node [midway, above right, font = \scriptsize] {$n_f$}}]]
%
[$\mathcal{T}(\Sigma)$ [ \ \ \ , no edge]] 
]
%\draw[-,dotted](1)..(i);
\end{forest}};
%
\node (iff) at (0,1.2) {$\xLeftrightarrow{\FH \vdash \FCS_i}$};
%
\node (right) at (3,0) {
\begin{forest}
[$\vdash$
[$\FHS_i$
[$\mathcal{T}(\Upsilon_1)$, -->, edge label = {node [midway, above left, font = \scriptsize] {$1$}}]
%
[$\mathcal{T}(\Sigma)$, -->, edge label = {node [midway, right, font = \scriptsize] {$i$}}]
%
[$\mathcal{T}(\Upsilon_{n_f})$, edge label = {node [midway, above right, font = \scriptsize] {$n_f$}}]]
%
[$\mathcal{T}(\Sigma_i)$ [ \ \ \ , no edge]] 
]
\end{forest}};
\end{tikzpicture}
\end{center}
}}

\noindent meaning that applying a display postulates swaps the `$\vdash$' label with the label on the $i$-th coordinate of $\FH$, changing the node $\FH$ with its residue and in the antitone case it reverses the direction of the label `$\vdash$'. The thesis follows from the observations above.
\end{proof}

\textcolor{red}{For all $\Upsilon, \Upsilon'\in \mathsf{Str}$, we write $\Upsilon\triangleleft\Upsilon'$ when  $\mathcal{T}(\Upsilon)$ is a subtree of  $\mathcal{T}(\Upsilon')$. We also write $\Upsilon \triangleleft (\Pi\vdash \Sigma)$ when $\Upsilon\triangleleft \Pi$ or $\Upsilon\triangleleft \Sigma$.}\marginnote{AP: propongo questa in alternative. ADD: ok approvo.}


\iffalse
\begin{definition}
    Let $\Pi_1\vdash \Sigma_1$ and $\Pi_2 \vdash \Sigma_2$ be display-equivalent sequents. We write $\Pi_1 \triangleleft \Pi_2$ whenever $\Pi_{1}$ is a substructure of $\Pi_{2}$ -- i.e., if $\mathcal{T}(\Pi_2)$ contains a subtree displayable on the left such that, when put in display, is isomorphic to $\mathcal{T}(\Pi_1)$. We define $\Sigma_1 \triangleleft \Pi_2$, $\Pi_1 \triangleleft \Sigma_2$, and $\Sigma_1 \triangleleft \Sigma_2$ analogously.
\end{definition}

\textcolor{red}{Think of good examples...}
\fi
\marginnote{AP: proporrei di omettere la dim. ADD: lascio la scelta a voi, per me ormai e' chiaro che la tesi sia vera.}
\begin{lemma} \label{lem:four_possible_decompositions}
   If $\Pi_0 \vdash \Sigma_0 $ and $\Pi_1 \vdash \Sigma_1$ are display-equivalent, then, for every $0\leq i\leq 1$,  
    $\Pi_i \triangleleft \Pi_{1-i}$ iff $\Sigma_{1-i}\triangleleft \Sigma_i$, and
 $\Pi_i \triangleleft \Sigma_{1-i}$ iff $ \Pi_{1-i}\triangleleft\Sigma_{i}$, and $\Pi_i\triangleleft \Upsilon_{1-i}$ for some $i$.
   \textcolor{red}{
    \begin{center}
        \begin{tabular}{c c c}
             $1)\ \Pi_i \triangleleft \Pi_2,\ \Sigma_2 \triangleleft \Sigma_1$ & \quad\quad  & $2)\ \Pi_2 \triangleleft \Sigma_1,\ \Pi_1 \triangleleft \Sigma_2$ \\
             $3)\ \Pi_2 \triangleleft \Pi_1,\ \Sigma_1 \triangleleft \Sigma_2$ & & $4)\ \Sigma_2 \triangleleft \Pi_1,\ \Sigma_1 \triangleleft \Pi_2$ 
        \end{tabular}
    \end{center}
    }
\end{lemma}

\begin{proof}
    By Lemma~\ref{lem:tree_under_display_postulates}, the trees $\mathcal{T}(\Pi_1 \vdash \Sigma_1)$ and $\mathcal{T}(\Pi_2 \vdash \Sigma_2)$ are isomorphic up to labels. Let `$\vdash_1$' and `$\vdash_2$' denote the corresponding edges in the two trees. Four cases arise from the position and orientation of `$\vdash_2$' relative to `$\vdash_1$': if `$\vdash_2$'  is in $\Sigma_1$ with same (resp.~opposite) orientation, then case 1 (resp.~2) holds; if $\vdash_2$ is in $\Pi_1$, then case 3 (resp.~4) holds.
\end{proof}
%\begin{proof}
   % By virtue of Lemma \ref{lem:tree_under_display_postulates}, the trees $\mathcal{T}(\Pi_1 \vdash \Sigma_1)$ and $\mathcal{T}(\Pi_2 \vdash \Sigma_2)$ are isomorphic once we remove all their labels. Consider the position of the edge labeled `$\vdash$' in $\mathcal{T}(\Pi_2 \vdash \Sigma_2)$ relative to the edge with the same label in $\mathcal{T}(\Pi_1 \vdash \Sigma_1)$ (we temporarily denote it as `$\vdash_2$' and `$\vdash_1$', respectively), four different cases are possible. If `$\vdash_2$' is inside $\Sigma_1$ facing the same (resp.~opposite) direction as `$\vdash_1$', then case $1$ (resp. case $2$) of the thesis holds, while if `$\vdash_2$' is inside $\Pi_1$ facing the same (resp.~opposite) direction as `$\vdash_1$', then case $3$ (resp. case $4$) of the thesis holds.
%\end{proof}
\marginnote{AP: questa non e' una definizione, e' solo una notazione}
\begin{dfn}
    Suppose a left structure $\Pi$ in a sequent $\Pi\vdash\Sigma$ contains a substructure that once displayed to the left (resp.~right) becomes $X$. If $Y$ is a left structure, we define $\Pi\{Y/X\}^{pre}\vdash \Sigma$ (resp.~$\Pi\{Y/X\}^{suc}\vdash \Sigma$) as the sequent obtained from $\Pi\vdash\Sigma$ after putting $X$ in display, substitute it with $Y$, and finally reverse all the previous display moves. The substitutions involving $\Sigma$ are defined analogously.
\end{dfn}
\marginnote{AP: propongo questa in alternative. ADD: Approvo.}
\textcolor{red}{For any sequent $\Pi\vdash\Sigma$  and all $\Pi', \Pi''\in \mathsf{Str}_{\mathcal{F}}$ (resp.~$\Sigma', \Sigma''\in \mathsf{Str}_{\mathcal{G}}$), if $\Pi'\triangleleft (\Pi\vdash \Sigma)$ (resp.~$\Sigma'\triangleleft (\Pi\vdash \Sigma)$) we let $(\Pi\vdash \Sigma)[\Pi''/\Pi']^{pre}$ (resp.~$(\Pi\vdash \Sigma)[\Sigma''/\Sigma']^{succ}$) denote the sequent whose generation tree is obtained by replacing  $\mathcal{T}(\Pi')$ (resp.~$\mathcal{T}(\Sigma')$) by $\mathcal{T}(\Pi'')$ (resp.~$\mathcal{T}(\Sigma'')$) as a subtree of $\mathcal{T}(\Pi\vdash\Sigma)$. In what follows, to indicate on which side of the sequent the replacement occurs, we will also use notational variants such as  $\Pi[\Pi''/\Pi']^{prec}\vdash \Sigma$, $\Pi[\Sigma''/\Sigma']^{suc}\vdash \Sigma$, $\Pi\vdash \Sigma[\Pi''/\Pi']^{prec}$, and $\Pi\vdash \Sigma[\Sigma''/\Sigma']^{suc}$.}
